Leveraging Unlabeled Data to Predict Out-of-Distribution Performance

Real-world machine learning deployments are characterized by mismatches between the source (training) and target (test) distributions that may cause performance drops. In this work, we investigate methods for predicting the target domain accuracy using only labeled source data and unlabeled target data. We propose Average Thresholded Confidence (ATC), a practical method that learns a threshold on the model's confidence, predicting accuracy as the fraction of unlabeled examples for which model confidence exceeds that threshold. ATC outperforms previous methods across several model architectures, types of distribution shifts (e.g., due to synthetic corruptions, dataset reproduction, or novel subpopulations), and datasets (Wilds, ImageNet, Breeds, CIFAR, and MNIST). In our experiments, ATC estimates target performance $2$-$4\times$ more accurately than prior methods. We also explore the theoretical foundations of the problem, proving that, in general, identifying the accuracy is just as hard as identifying the optimal predictor and thus, the efficacy of any method rests upon (perhaps unstated) assumptions on the nature of the shift. Finally, analyzing our method on some toy distributions, we provide insights concerning when it works. Code is available at https://github.com/saurabhgarg1996/ATC_code/.

==> ICLR 2022_ Prediction Accuracy on OOD Data/sections/00_abstract.tex <==

Real-world machine learning deployments are characterized by mismatches between the source (training) and target (test) distributions that may cause performance drops. In this work, we investigate methods for predicting the target domain accuracy using only labeled source data and unlabeled target data. We propose Average Thresholded Confidence (ATC),
a practical method that learns a \emph{threshold} on the model's confidence, predicting accuracy as the fraction of unlabeled examples for which model confidence exceeds that threshold. ATC outperforms previous methods across several model architectures, types of distribution shifts 
(e.g., due to synthetic corruptions, dataset reproduction, or novel subpopulations), and datasets (\update{\textsc{Wilds}}, ImageNet, \breeds, CIFAR, and MNIST). In our experiments, ATC estimates target performance 
$2\text{--}4\times$ more accurately than prior methods. 
We also explore the theoretical foundations of the problem,
proving that, in general, identifying the accuracy
is just as hard as identifying the optimal predictor
and thus, the efficacy of any method
rests upon (perhaps unstated) assumptions 
on the nature of the shift. 
Finally, analyzing our method on some toy distributions,
we provide insights concerning when it works\footnote{Code is available at \url{https://github.com/saurabhgarg1996/ATC_code}.}.






        






==> ICLR 2022_ Prediction Accuracy on OOD Data/sections/01_intro.tex <==

Machine learning models deployed in the real world 
typically encounter examples 
from previously unseen distributions. 
While the IID assumption enables us to
evaluate models using held-out data 
from the \emph{source} distribution 
(from which training data is sampled),
this estimate is no longer valid
in presence of a distribution shift.
Moreover, under such shifts,
model accuracy tends to degrade
\citep{szegedy2013intriguing, recht2019imagenet,wilds2021}.
Commonly, the only data
available to the practitioner
are a labeled training set (source)
and unlabeled deployment-time data which makes the problem more difficult.
In this setting, detecting shifts 
in the distribution of covariates
is known to be possible (but difficult)
in theory~\citep{ramdas2015decreasing},
and in practice~\citep{rabanser2018failing}.
However, producing an optimal predictor 
using only labeled source and unlabeled target data
is well-known to be impossible absent further assumptions~\citep{ben2010impossibility,lipton2018detecting}. %


Two vital questions that remain are:
(i) the precise conditions under which 
we can estimate a classifier's target-domain accuracy;
and (ii) which methods are most practically useful.
To begin, the straightforward way 
to assess the performance 
of a model under distribution shift
would be to collect labeled (target domain) examples 
and then to evaluate the model on that data. 
However, collecting fresh labeled data 
from the target distribution 
is prohibitively expensive and time-consuming, 
especially if the target distribution is non-stationary. 
Hence, instead of using labeled data,
we aim to use 
unlabeled data from the target 
distribution, that is comparatively abundant, to predict model performance. 
Note that in this work, our focus 
is \emph{not} to improve performance on the target 
but, rather, to estimate the accuracy on the target for a given classifier.

Recently, numerous methods have been proposed 
for this purpose~\citep{deng2021labels,chen2021mandoline,jiang2021assessing,deng2021does,guillory2021predicting}. 
These methods either require calibration on the target domain 
to yield consistent estimates~\citep{jiang2021assessing,guillory2021predicting} 
or additional labeled data 
from several target domains 
to learn a linear regression function
on a distributional distance that then 
predicts model performance~\citep{deng2021does,deng2021labels,guillory2021predicting}. 
However, methods that require calibration 
on the target domain typically yield poor estimates 
since deep models trained and calibrated on 
source data are not, in general, calibrated on a 
(previously unseen) target domain~\citep{ovadia2019can}. 
Besides, methods that leverage  
labeled data from target domains rely
on the fact that unseen target domains exhibit strong 
linear correlation with seen target domains 
on the underlying distance measure and, hence, 
can be rendered ineffective when 
such target domains with labeled data 
are unavailable (in \secref{sec:exp_results} 
we demonstrate such a failure on a real-world 
distribution shift problem). 
Therefore, throughout the paper,
we assume access to labeled source data 
and only unlabeled data from target domain(s).   


\begin{figure*}[t!]
    \centering 
    \includegraphics[width=\linewidth]{figures/intro_fig_final.pdf}
    \vspace{-10pt}
    \caption{\emph{Illustration of our proposed method ATC.} {} \textbf{Left}: 
    using source domain validation data, 
    we identify a \emph{threshold}
    on a score (e.g. negative entropy)
    computed on model confidence
    such that fraction of examples above the threshold
    matches the validation set accuracy. 
    ATC estimates accuracy on unlabeled target data 
    as the fraction of examples 
    with the score above the threshold.
    Interestingly, this threshold yields accurate estimates
    on a wide set of target distributions 
    resulting from natural and synthetic shifts.{} 
    \textbf{Right}: \update{Efficacy of ATC 
    over previously proposed approaches on our testbed
    with a post-hoc calibrated model.} 
    To obtain errors on the same scale, 
    we rescale all errors with Average Confidence (AC) error. 
    Lower estimation error is better.
    See \tabref{table:error_estimation} for exact numbers 
    and comparison on various types of distribution shift. 
    See \secref{sec:exp} for details on our testbed.}
    \label{fig:intro}
    \vspace{-10pt}
  \end{figure*}


 
In this work, we first show that
{absent assumptions 
on the source classifier or the nature of the shift,
no method of estimating accuracy will work generally}
(even in non-contrived settings).
To estimate accuracy on target domain \emph{perfectly},  
we highlight that even given perfect knowledge 
of the labeled source distribution (i.e., $p_s(x,y)$) 
and unlabeled target distribution (i.e., $p_t(x)$),
we need restrictions on the nature of the shift 
such that we can uniquely identify 
the target conditional $p_t(y|x)$.  
Thus, in general, identifying the accuracy of the classifier
is as hard as identifying the optimal predictor.

Second, motivated by the superiority
of methods that use maximum softmax 
probability (or logit) of a model 
for Out-Of-Distribution (OOD) 
detection~\citep{hendrycks2016baseline,hendrycks2019scaling}, 
we propose a simple method 
that leverages softmax probability to
predict model performance.  
Our method, {Average Thresholded Confidence} (ATC), 
learns a threshold on a score 
(e.g., maximum confidence or negative entropy) 
of model confidence on validation source data 
and predicts target domain accuracy
as the fraction of unlabeled target points 
that receive a score above that threshold. 
ATC selects a threshold on validation source data 
such that the fraction of source examples   
that receive the score  
above the threshold match the 
accuracy of those examples.  
Our primary contribution in ATC
is the proposal of obtaining the threshold 
and observing its efficacy 
on (practical) accuracy estimation.  
Importantly, our work takes a step forward 
in positively answering the question raised 
in \citet{deng2021labels,deng2021does} 
about a practical strategy 
to select a threshold that enables 
accuracy prediction with thresholded model confidence. 


ATC is simple to implement with existing frameworks, 
compatible with arbitrary model classes, 
and dominates other contemporary methods.
\update{Across several model architectures on a 
range of benchmark vision and 
language datasets, 
we verify that ATC outperforms
prior methods by at least $2$--$4\times$ in 
predicting target accuracy 
on a variety of distribution shifts.}
In particular, we consider 
shifts due to common corruptions (e.g., ImageNet-C), 
natural distribution shifts due to 
dataset reproduction (e.g., ImageNet-v2, ImageNet-R), 
shifts due to novel
subpopulations (e.g., \textsc{Breeds}), 
and distribution shifts faced in the wild (e.g., \textsc{Wilds}). 

As a starting point for theory development, 
we investigate ATC on a simple toy model
that models distribution shift 
with varying proportions of the population 
with spurious features,
as in \citet{nagarajan2020understanding}. 
Finally, we note that  
although ATC achieves 
superior performance in 
our empirical evaluation, like all methods, 
it must fail (returns inconsistent estimates) 
on certain types of distribution shifts,
per our impossibility result.


























 









==> ICLR 2022_ Prediction Accuracy on OOD Data/sections/02_prior.tex <==
\textbf{Out-of-distribution detection. {} {}} 
The main goal of OOD detection is 
to identify previously unseen examples, 
i.e., samples out of the support
 of training distribution.  
To accomplish this, modern methods
utilize confidence or features learned 
by a deep network  trained 
on some source data. 
\citet{hendrycks2016baseline,geifman2017selective}
used the confidence score 
of an (already) trained deep model
to identify OOD points. 
\citet{lakshminarayanan2016simple} use entropy 
of an ensemble model to evaluate prediction 
uncertainty on OOD points. 
To improve OOD detection with model confidence, 
\citet{liang2017enhancing} propose to use 
temperature scaling and input perturbations.  
% 
\citet{jiang2018trust} propose to use 
scores based on the relative 
distance of the predicted class 
to the second class. Recently, 
residual flow-based methods 
were used to obtain a density model 
for OOD detection~\citep{zhang2020hybrid}. 
\citet{ji2021predicting} proposed a method 
based on subfunction error bounds to compute 
unreliability per sample. Refer to 
\citet{ovadia2019can,ji2021predicting} for an overview 
and comparison of methods for prediction uncertainty 
on OOD data. 
% 

\textbf{Predicting model generalization. {} {}}
Understanding generalization capabilities 
of overparameterized models on in-distribution 
data using conventional machine learning tools 
has been a focus of a long line of work; 
representative research includes~\citet{neyshabur2015norm,neyshabur2017exploring,neyshabur2017implicit,neyshabur2018role,dziugaite2017computing,bartlett2017spectrally,zhou2018non,long2019generalization, nagarajan2019deterministic}. 
% 
At a high level, this line of research 
bounds the generalization gap directly 
with complexity measures calculated on
the trained model.
% 
However, these bounds typically remain 
numerically loose relative to the true 
generalization error~\citep{zhang2016understanding,nagarajan2019uniform}. 
% 
On the other hand, another line of research 
departs from complexity-based approaches to 
use unseen unlabeled data to predict in-distribution 
generalization~\citep{platanios2016estimating,platanios2017estimating,garg2021ratt,jiang2021assessing}.
 

Relevant to our work are methods for predicting 
the error of a classifier on OOD data 
based on unlabeled data from the target (OOD) domain. 
%
These methods can be characterized into two broad categories: 
(i) Methods which explicitly predict correctness of the model 
on individual unlabeled points~\citep{deng2021labels, jiang2021assessing,deng2021does, chen2021detecting}; and
(ii) Methods which directly obtain an estimate of error with unlabeled OOD data 
without making a point-wise prediction~\citep{chen2021mandoline,guillory2021predicting,chuang2020estimating}. 


To achieve a consistent estimate of the target accuracy, 
~\citet{jiang2021assessing,guillory2021predicting} require
calibration on target domain. 
However, these methods typically yield poor estimates 
as deep models trained and calibrated on some source data 
are seldom calibrated on previously
unseen domains~\citep{ovadia2019can}.  
%
Additionally, \citet{deng2021labels,guillory2021predicting} 
derive model-based distribution statistics 
on unlabeled target set that correlate 
with the target accuracy and propose 
to use a subset of \emph{labeled} target 
domains to learn a (linear) regression 
function that predicts model performance. 
However, there are two drawbacks with this approach: 
(i) the correlation of these distribution 
statistics can vary substantially as we consider 
different nature of shifts 
(refer to \secref{sec:exp_results},
where we empirically demonstrate this failure);
%  
(ii) even if there exists a (hypothetical) 
statistic with strong correlations, 
obtaining labeled target domains (even simulated ones) 
with strong correlations would require significant
\emph{a priori} knowledge about the nature of shift
that, in general, might not be available 
before models are deployed in the wild.  
% Moreover, the shifts also leak some 
% information about the shifts occurring in practice. 
Nonetheless, in our work, we only assume access 
to labeled data from the source domain presuming 
no access to labeled target domains or 
information about how to simulate them. 
% 

Moreover, unlike the parallel work of \citet{deng2021does}, 
we do not focus on methods
that alter the training on source data 
to aid accuracy prediction on the target data. 
%
\citet{chen2021mandoline} propose an 
importance re-weighting based approach 
that leverages (additional) information 
about the axis along which distribution 
is shifting in form of ``slicing functions''. 
%
In our work, we make comparisons with 
importance re-weighting 
baseline from \citet{chen2021mandoline} 
as we do not have any additional 
information about the axis along which 
the distribution is shifting. 

==> ICLR 2022_ Prediction Accuracy on OOD Data/sections/03_setup.tex <==
\textbf{Notation.} By $\enorm{\cdot}$, 
and $\inner{\cdot}{\cdot}$
we denote the Euclidean norm
and inner product,
respectively.
For a vector $v\in \Real^d$, 
we use $v_j$ to denote its $j^\text{th}$ entry, 
and for an event $E$ we let $\indict{E}$ 
denote the binary indicator of the event.

Suppose we have a multi-class classification problem
with the input domain $\calX \subseteq \Real^d$ 
and label space $\calY = \{1, 2, \ldots, k\}$. For 
binary classification, 
we use $\calY = \{0,1\}$. 
By $\calD^\train$ and $\calD^\test$, 
we denote source and target distribution 
over $\calX \times \calY$. For distributions 
$\calD^\train$ and $\calD^\test$, we 
define $p_\train$ or $p_\test$ as the
corresponding probability density (or mass) 
functions. A dataset 
$S \defeq \{(x_i, y_i)\}_{i=1}^n \sim (\calD^\train)^n$
contains $n$ points sampled i.i.d. from $\calD^\train$.
Let $\calF$ be a class of hypotheses 
mapping $\calX$ to $\Delta^{k-1}$ where $\Delta^{k-1}$ is a simplex in $k$ dimensions. 
Given a classifier $f \in \calF$ and datum $(x, y)$,
we denote the 0-1 error 
(i.e., classification error)
on that point by 
$\error(f(x), y) \defeq \indict{ y\not\in \argmax_{j\in\calY} f_j(x) }$. 
Given a model $f \in \calF$, 
our goal in this work is to understand the performance 
of $f$ on $\calD^\test$ without access to 
labeled data from $\calD^\test$. Note that our goal
is not to adapt the model to the target data.  
Concretely, we aim to predict accuracy of $f$ 
on $\calD^\test$. Throughout this paper, 
we assume we have access to the following: 
(i) model $f$; (ii) previously-unseen (validation) data 
from $\calD^\train$; and
(iii) unlabeled data from target distribution $\calD^\test$. 

\vspace{-7pt}
\subsection{Accuracy Estimation: Possibility and Impossibility Results}
\vspace{-3pt}

First, we investigate the question 
of when it is possible 
to estimate the target accuracy
of an arbitrary classifier,
even given knowledge of the full
source distribution $p_s(x,y)$ 
and target marginal $p_t(x)$. 
Absent assumptions on the nature of shift,
estimating target accuracy is impossible. 
Even given access to $p_s(x,y)$ and $p_t(x)$,
the problem is fundamentally 
unidentifiable 
because $p_t(y|x)$ can shift arbitrarily. 
In the following proposition, 
we show that absent assumptions 
on the classifier $f$ 
(i.e., when $f$ can be any classifier 
in the space of all classifiers on $\calX$), 
we can estimate accuracy on the 
target data iff assumptions
on the nature of the shift,
together with $p_s(x, y)$ and $p_t(x)$,
uniquely identify the (unknown) target 
conditional $p_t(y|x)$. 
We relegate proofs from this section to 
\appref{app:proof_setup}. %

\begin{proposition} \label{prop:characterization}
Absent further assumptions,
accuracy on the 
target is identifiable 
iff $p_t(y|x)$ is uniquely identified 
given $p_s(x, y)$ and $p_t(x)$. 
\end{proposition}

\propref{prop:characterization} states that 
we need enough constraints on nature of shift 
such that $p_s(x, y)$ and $p_t(x)$
identifies unique $p_t(y|x)$. 
It also states that under some assumptions 
on the nature of the shift, 
we can hope to estimate 
the model's accuracy on target data. 
We will illustrate this
on two common assumptions 
made in domain adaptation literature:
(i) covariate shift~\citep{heckman1977sample,shimodaira2000improving} 
and (ii) label shift~\citep{saerens2002adjusting,zhang2013domain,lipton2018detecting}. 
Under covariate shift assumption, 
that the target marginal support $\textbf{supp}(p_t(x))$
is a subset of the source marginal support $\textbf{supp}(p_s(x))$
and that the conditional distribution of labels given inputs 
does not change within support,
i.e.,  $p_s(y|x) = p_t(y|x)$,
which, trivially, identifies 
a unique target conditional $p_t(y|x)$. 
Under label shift, the reverse holds, i.e.,
the class-conditional distribution 
does not change ($p_s(x|y) = p_t(x|y)$)
and, again, information about $p_t(x)$ uniquely determines 
the target conditional $p_t(y|x)$~\citep{lipton2018detecting,garg2020unified}. 
In these settings, one can estimate 
an arbitrary classifier's accuracy 
on the target domain either 
by using importance re-weighting 
with the ratio $p_t(x)/p_s(x)$
in case of covariate shift 
or by using importance re-weighting 
with the ratio $p_t(y)/p_s(y)$ 
in case of label shift. 
While importance ratios in the former case
can be obtained directly 
when $p_t(x)$ and $p_s(x)$ are known, 
the importance ratios in the latter case 
can be obtained by using techniques from ~\citet{saerens2002adjusting,lipton2018detecting,azizzadenesheli2019regularized, alexandari2019adapting}. 
In \appref{app:estimate_label_covariate},%
we explore accuracy estimation 
in the setting of these shifts and present extensions 
to generalized notions of label shift~\citep{tachet2020domain} 
and covariate shift~\citep{rojas2018invariant}. 

As a corollary of \propref{prop:characterization}, 
we now present a simple impossibility result,
demonstrating that no single method can work 
for all families of distribution shift. 

\begin{corollary} \label{corollary:impossible}
Absent assumptions on the classifier $f$, 
no method of estimating accuracy will 
work in all scenarios, i.e., for different 
nature of distribution shifts. 
\end{corollary}
Intuitively, this result states that 
every method of estimating accuracy on 
target data is tied up with some assumption
on the nature of the shift and might not 
be useful for estimating accuracy under a  
different assumption on the nature of the shift.
For illustration, consider a setting 
where we have access to distribution 
$p_s(x, y)$ and $p_t(x)$. 
Additionally, assume 
that the distribution can shift 
only due to covariate shift or
label shift without any knowledge 
about which one. 
Then \corollaryref{corollary:impossible} 
says that it is impossible to have a single 
method that will simultaneously for both label 
shift and covariate shift as in the following example
(we spell out the details in \appref{app:proof_setup}):%

\textbf{Example 1.}
Assume binary classification with  
$p_s(x) = \alpha \cdot \phi(\mu_1) + (1-\alpha)\cdot \phi(\mu_2)$, 
$p_s(x|y=0) = \phi(\mu_1)$, $p_s(x|y=1) =  \phi(\mu_2)$,  
and 
$p_t(x) = \beta\cdot \phi(\mu_1) + (1-\beta) \cdot \phi(\mu_2)$ 
where $\phi(\mu) = \calN(\mu, 1)$, $\alpha,\beta \in (0,1)$,
and $\alpha \ne \beta$. 
Error of a classifier $f$ on target data is given by 
$\calE_1=\Expt{(x,y)\sim p_s(x,y)}{\frac{p_t(x)}{p_s(x)} \indict{f(x)\ne y}}$
under covariate shift and by 
$\calE_2=\Expt{(x,y)\sim p_s(x,y)}{\left(\frac{\beta}{\alpha}\indict{y=0} + \frac{1-\beta}{1-\alpha}\indict{y=1} \right)\indict{f(x)\ne y}}$
under label shift. 
In \appref{app:proof_setup},
we show that $\calE_1 \ne \calE_2$ for all $f$. 
Thus, given access to $p_s(x,y)$, and $p_t(x)$, 
any method that consistently estimates 
error of a classifer under covariate shift will give an
incorrect estimate of error 
under label shift and vice-versa.   
The reason is that the same $p_t(x)$ and $p_s(x,y)$
can correspond to error $\calE_1$ (under covariate shift)
or error $\calE_2$ (under label shift) 
and determining which scenario one faces
requires further assumptions on the nature of shift. 




==> ICLR 2022_ Prediction Accuracy on OOD Data/sections/04_proposed_method.tex <==
In this section, we present our method ATC 
that leverages a black box classifier $f$ 
and (labeled) validation source data to 
predict accuracy on target domain given
access to unlabeled target data. 
Throughout the discussion, we assume 
that the classifier $f$ is fixed.  

Before presenting our method, 
we introduce some terminology. 
Define a score function 
$s: \Delta^{k-1} \to \Real$ 
that takes in the softmax prediction
of the function $f$ 
and outputs a scalar. 
We want a score function 
such that if the score function 
takes a high value at a datum $(x,y)$ 
then $f$ is likely to be correct. 
In this work, we explore two such 
score functions: 
(i) Maximum confidence, i.e., 
$s(f(x)) = \underset{j \in \calY}{\max} f_j(x)$; 
and (ii) Negative Entropy, i.e.,
$s(f(x)) = \sum_j f_j(x) \log(f_j(x))$.
Our method identifies a threshold $t$ 
on source data $\calD^\train$
such that the expected number of points 
that obtain a score less than $t$ 
match the error of $f$ on $\calD^\train$, i.e., 
\begin{align}
    \Expt{x \sim \calD^\train }{\indict{ s(f(x)) < t}}  = \Expt{(x,y) \sim \calD^\train}{\indict{ \argmax_{j\in \out} f_j(x) \ne y}} \,, 
    \label{eq:ATC_thres}
\end{align}
and then our error estimate $\text{ATC}_{D^\test}(s)$
on the target domain $\calD^\test$ is given 
by the expected number of target points
that obtain a score less than $t$, i.e., 
\begin{align}
    \text{ATC}_{\calD^\test}(s) =  \Expt{x \sim \calD^\test}{\indict{ s(f(x)) < t}}  \,.
    \label{eq:ATC_pred}
\end{align}
In short, in \eqref{eq:ATC_thres},
ATC selects a threshold on the score function 
such that the error in the source domain 
matches the expected number of points 
that receive a score below $t$ 
and in \eqref{eq:ATC_pred},
ATC predicts error on the target domain 
as the fraction of unlabeled points 
that obtain a score below that threshold $t$. 
Note that, in principle, there exists 
a different threshold $t^\prime$
on the target distribution $\calD^\test$ 
such that \eqref{eq:ATC_thres}
is satisfied on $\calD^\test$. 
However, in our experiments,
the same threshold performs remarkably well.
The main empirical contribution of our work 
is to show that the threshold obtained with 
\eqref{eq:ATC_thres} might be used effectively
in condunction with modern deep networks
in a wide range of settings
to estimate error on the target data.
In practice, to obtain the threshold with ATC, 
we minimize the difference between the 
expression on two sides of \eqref{eq:ATC_thres}
using finite samples. 
In the next section,  
we show that ATC precisely
predicts accuracy on the OOD data  
on the desired line $y=x$. 
In \appref{app:interpretation}, %
we discuss an alternate 
interpretation of the method and make 
connections with OOD detection methods. 




==> ICLR 2022_ Prediction Accuracy on OOD Data/sections/05_exp.tex <==


\begin{figure}[t]
\vspace{-20pt}
    \centering
    \subfigure{\includegraphics[width=0.32\linewidth]{figures/CIFAR10.pdf}} \hfil
    \subfigure{\includegraphics[width=0.32\linewidth]{figures/ImageNet200.pdf}} \hfil   
    \subfigure{\includegraphics[width=0.32\linewidth]{figures/Living17.pdf}} 
    \vspace{-12pt}
    \caption{\emph{Scatter plot of predicted accuracy versus (true) OOD accuracy.}
    Each point denotes a different OOD dataset, 
    all evaluated with the same DenseNet121 model.
    We only plot the best three methods. 
    With ATC (ours), we refer to ATC-NE. 
    We observe that ATC significantly outperforms other methods 
    and with ATC, we recover the desired line $y=x$ with a robust linear fit. 
    Aggregated estimation error in \tabref{table:error_estimation} 
    and plots for other datasets and architectures in \appref{app:results}.} 
    \vspace{-15pt}
    \label{fig:scatter_plot}
  \end{figure}  
  

We now empirical evaluate 
ATC and compare it with existing methods. 
In each of our main experiment, 
keeping the underlying model fixed, 
we vary target datasets and make a 
prediction of the target accuracy 
with various methods given access to 
only unlabeled data from the target. 
Unless noted otherwise, all models are  
trained only on samples from the source 
distribution with the main exception of pre-training
on a different distribution. 
We use labeled examples from the 
target distribution to only obtain 
true error estimates. 

\textbf{Datasets. {}} First, we consider 
synthetic shifts induced due to 
different visual corruptions (e.g., shot noise, 
motion blur etc.) under 
ImageNet-C~\citep{hendrycks2019benchmarking}. 
Next, we consider natural shifts 
due to differences in the data 
collection process of ImageNet~\citep{russakovsky2015imagenet}, 
e.g, ImageNetv2~\citep{recht2019imagenet}. 
We also consider images with artistic 
renditions of object classes, i.e., 
ImageNet-R~\citep{hendrycks2021many} 
and ImageNet-Sketch~\citep{wang2019learning}. 
Note that renditions dataset only contains 
a subset $200$ 
classes from ImageNet. 
To include renditions dataset
in our testbed, we include results on 
ImageNet restricted 
to these $200$ classes (which we call 
ImageNet-200) along with full ImageNet. 

Second, we consider \textsc{Breeds}~\citep{santurkar2020breeds} 
to assess robustness to subpopulation shifts, in particular, 
to understand how accuracy estimation 
methods behave when novel subpopulations 
not observed during training are introduced. 
\textsc{Breeds} leverages class hierarchy 
in ImageNet to create 4 datasets \textsc{Entity-13}, \textsc{Entity-30},
\textsc{Living-17}, \textsc{Non-living-26}. We focus on 
natural and synthetic shifts as in ImageNet on same and different
subpopulations in BREEDs. 
\update{Third, from \textsc{Wilds}~\citep{wilds2021} benchmark, we consider 
FMoW-\textsc{Wilds}~\citep{christie2018functional}, 
RxRx1-\textsc{Wilds}~\citep{taylor2019rxrx1}, 
Amazon-\textsc{Wilds}~\citep{ni2019justifying}, 
CivilComments-\textsc{Wilds}~\citep{borkan2019nuanced}
to consider distribution shifts faced in the wild.
}

Finally, similar to ImageNet, 
we consider (i) synthetic shifts (CIFAR-10-C) due to 
common corruptions; and (ii) natural shift 
(i.e., CIFARv2~\citep{recht2018cifar})
on CIFAR-10~\citep{krizhevsky2009learning}.  
On CIFAR-100, we just have  
synthetic shifts due to common corruptions. 
For completeness, we also consider natural shifts 
on MNIST~\citep{lecun1998mnist}
as in the prior work~\citep{deng2021labels}. 
We use three real shifted datasets, i.e., USPS~\citep{hull1994database},
SVHN~\citep{netzer2011reading} and QMNIST~\citep{qmnist-2019}. 
We give a detailed overview of our setup in \appref{app:dataset}.  %

\textbf{Architectures and Evaluation. {}{}}
\update{For ImageNet, \textsc{Breeds}, CIFAR, FMoW-\textsc{Wilds}, 
RxRx1-\textsc{Wilds}
datasets, we use DenseNet121~\citep{huang2017densely} 
and ResNet50~\citep{he2016deep} architectures. 
For Amazon-\textsc{Wilds} and CivilComments-\textsc{Wilds},
we fine-tune a  DistilBERT-base-uncased~\citep{Sanh2019DistilBERTAD} model. }
For MNIST, we train a fully 
connected multilayer perceptron.  
We use standard training
with benchmarked hyperparameters. 
To compare methods, we report average 
absolute difference between 
the true accuracy on the target data and the 
estimated accuracy on the same unlabeled examples. 
We refer to this metric as Mean Absolute estimation Error~(MAE). 
Along with MAE, we also show scatter plots 
to visualize performance at individual target sets. 
Refer to \appref{app:exp_setup} for additional %
details on the setup.   


\begin{table}[t]
    \begin{adjustbox}{width=\columnwidth,center}
    \centering
    \tabcolsep=0.12cm
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{@{}*{13}{c}@{}}
    \toprule
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Shift} & \multicolumn{2}{c}{IM} & \multicolumn{2}{c}{AC} & \multicolumn{2}{c}{DOC} & GDE & \multicolumn{2}{c}{ATC-MC (Ours)} & \multicolumn{2}{c}{ATC-NE (Ours)} \\
    & & Pre T & Post T & Pre T & Post T  & Pre T & Post T & Post T & Pre T & Post T & Pre T & Post T \\
    \midrule
    \multirow{2}{*}{\parbox{1.2cm}{CIFAR10} }  & Natural & $6.60$ &$5.74$ &$9.88$ &$6.89$ &$7.25$ &$6.07$ &$4.77$ &$3.21$ &$3.02$ &$2.99$ & $\bf 2.85$   \\
    & Synthetic & $12.33$ &$10.20$ &$16.50$ &$11.91$ &$13.87$ &$11.08$ &$6.55$ &$4.65$ &$4.25$ &$4.21$ &$\bf 3.87$ \\ 
    \midrule 
    CIFAR100 & Synthetic & $13.69$ &$11.51$ &$23.61$ &$13.10$ &$14.60$ &$10.14$ &$9.85$ &$5.50$ &$\bf 4.75$ &$\bf 4.72$ &$4.94$ \\
    \midrule  
    \multirow{2}{*}{\parbox{1.8cm}{ImageNet200} }  & Natural & $12.37$ &$8.19$ &$22.07$ &$8.61$ &$15.17$ &$7.81$ &$5.13$ &$4.37$ &$2.04$ &$3.79$ & $\bf 1.45$ \\
    & Synthetic & $19.86$ &$12.94$ &$32.44$ &$13.35$ &$25.02$ &$12.38$ &$5.41$ &$5.93$ &$3.09$ &$5.00$ &$\bf 2.68$  \\ 
    \midrule 
    \multirow{2}{*}{\parbox{1.8cm}{\centering ImageNet} }  & Natural &
    $7.77$ &$6.50$ &$18.13$ &$6.02$ &$8.13$ &$5.76$ &$6.23$ &$3.88$ &$2.17$ &$2.06$ &$\bf 0.80$ \\
        & Synthetic &$13.39$ &$10.12$ &$24.62$ &$8.51$ &$13.55$ &$7.90$ &$6.32$ &$3.34$ &$\bf 2.53$ &$\bf 2.61$ &$4.89$ \\ 
    \midrule 
    FMoW-\textsc{wilds} & Natural & $5.53$ &$4.31$ &$33.53$ &$12.84$ &$5.94$ &$4.45$ &$5.74$ &$3.06$ &$\bf 2.70$ &$3.02$ &$\bf 2.72$  \\
    \midrule 
    RxRx1-\textsc{wilds} & Natural & $5.80$ &$5.72$ &$7.90$ &$4.84$ &$5.98$ &$5.98$ &$6.03$ &$4.66$ &$\bf 4.56$ &$\bf 4.41$ &$\bf 4.47$ \\
    \midrule 
    Amazon-\textsc{wilds} & Natural & $2.40$ &$2.29$ &$8.01$ &$2.38$ &$2.40$ &$2.28$ &$17.87$ &$1.65$ &$\bf 1.62$ &$ \bf 1.60$ &$\bf 1.59$ \\
    \midrule 
    CivilCom.-\textsc{wilds} & Natural & $12.64$ &$10.80$ &$16.76$ &$11.03$ &$13.31$ &$10.99$ &$16.65$ & \multicolumn{4}{c}{$\bf 7.14$} \\
    \midrule 
    MNIST & Natural &$18.48$ &$15.99$ &$21.17$ &$14.81$ &$20.19$ &$14.56$ &$24.42$ &$5.02$ &$\bf 2.40$ &$3.14$ &$3.50$ \\
    \midrule 
    \multirow{2}{*}{\parbox{1.8cm}{\textsc{Entity-13}} } & Same & $16.23$ &$11.14$ &$24.97$ &$10.88$ &$19.08$ &$10.47$ &$10.71$ &$5.39$ &$\bf 3.88$ &$4.58$ &$4.19$ \\
    & Novel & $28.53$ &$22.02$ &$38.33$ &$21.64$ &$32.43$ &$21.22$ &$20.61$ &$13.58$ &$10.28$ &$12.25$ &$\bf 6.63$ \\
    \midrule 
    \multirow{2}{*}{\parbox{1.8cm}{\textsc{Entity-30}}} & Same & $18.59$ &$14.46$ &$28.82$ &$14.30$ &$21.63$ &$13.46$ &$12.92$ &$9.12$ &$\bf 7.75$ &$8.15$ &$ \bf 7.64$ \\
    & Novel & $32.34$ &$26.85$ &$44.02$ &$26.27$ &$36.82$ &$25.42$ &$23.16$ &$17.75$ &$14.30$ &$15.60$ &$\bf 10.57$  \\
    \midrule
    \multirow{2}{*}{{\textsc{Nonliving-26}}} & Same & $18.66$ &$17.17$ &$26.39$ &$16.14$ &$19.86$ &$15.58$ &$16.63$ &$10.87$ &$\bf 10.24$ &$10.07$ &$\bf 10.26$ \\
    & Novel &$33.43$ &$31.53$ &$41.66$ &$29.87$ &$35.13$ &$29.31$ &$29.56$ &$21.70$ &$20.12$ &$19.08$ &$\bf 18.26$  \\ 
    \midrule 
    \multirow{2}{*}{\parbox{1.8cm}{\textsc{Living-17}}} & Same & $12.63$ &$11.05$ &$18.32$ &$10.46$ &$14.43$ &$10.14$ &$9.87$ &$4.57$ &$\bf  3.95$ &$\bf 3.81$ &$4.21$   \\
    & Novel & $29.03$ &$26.96$ &$35.67$ &$26.11$ &$31.73$ &$25.73$ &$23.53$ &$16.15$ &$14.49$ &$12.97$ &$\bf 11.39$ \\ 
    \bottomrule 
    \end{tabular}
  \end{adjustbox}  
    \vspace{-5pt}
    \caption{
    \emph{Mean Absolute estimation Error (MAE) results for different datasets in our setup grouped by the nature of shift.} 
    `Same' refers to same subpopulation shifts and `Novel' refers novel subpopulation shifts. \update{We include details about the target sets considered in each shift in \tabref{table:dataset}.} 
    Post T denotes use of TS calibration on source.  
    Across all datasets, we observe that ATC achieves superior performance (lower MAE is better).  
    \update{For language datasets, we use DistilBERT-base-uncased, for vision dataset we report results with DenseNet model with the exception of MNIST where we use FCN.} 
    We include results on other architectures in \appref{app:results}. 
    For GDE post T and pre T estimates match since TS doesn't alter the argmax prediction. \update{ Results reported by aggregating MAE numbers over $4$ different seeds. We include results with standard deviation values in \tabref{table:error_estimation_std}.}
    }\label{table:error_estimation}
    \vspace{-10pt}
\end{table}


\textbf{Methods {} {}} With ATC-NE, we denote ATC with negative entropy score function and with ATC-MC, 
we denote ATC with maximum confidence score function. 
For all methods, we implement \emph{post-hoc} calibration
on validation source data 
with Temperature Scaling (TS;~\citet{guo2017calibration}). 
Below we briefly discuss baselines methods 
compared in our work and relegate details to \appref{app:baselines}.  %
   

\emph{Average Confidence (AC). {}{}} Error is estimated as the expected value of the maximum softmax confidence  on the target data, i.e, $\AC_{\calD^\test} = \Expt{x \sim \calD^\test}{ \max_{j\in\calY} f_j(x)}$. 

\emph{Difference Of Confidence (DOC). {}{}} We estimate error on target by subtracting difference of confidences on source and target (as a surrogate to distributional distance~\citet{guillory2021predicting}) from the error on source distribution, i.e, $\DOC_{\calD^\test} = \Expt{x \sim \calD^\train}{ \indict{\argmax_{j\in\calY} f_j(x) \ne y}} + \Expt{x \sim \calD^\test}{ \max_{j\in\calY} f_j(x)} - \Expt{x \sim \calD^\train}{ \max_{j\in\calY} f_j(x)}$. This is referred to as DOC-Feat in \citep{guillory2021predicting}. 

\emph{Importance re-weighting (IM). {} {}} 
We estimate the error of the classifier 
with importance 
re-weighting of 0-1 error in the 
pushforward space 
of the classifier. 
This corresponds to \textsc{Mandolin} 
using one slice based on the underlying 
classifier confidence~\citet{chen2021mandoline}. 

\emph{Generalized Disagreement Equality (GDE). {} {}} 
Error is estimated as the expected disagreement of two models (trained on the same training set but with different randomization) on target data~\citep{jiang2021assessing}, i.e., $\GDE_{\calD^\test} = \Expt{x \sim \calD^\test}{\indict{f(x) \ne f^\prime(x)}}$ where $f$ and $f^\prime$ are the two models. Note that GDE requires two models trained independently, doubling the computational overhead while training. 


\vspace{-10pt}
\subsection{Results} \label{sec:exp_results}
\vspace{-5pt}

\begin{figure}[t]
\vspace{-10pt}
    \centering
    \subfigure{\includegraphics[width=0.3\linewidth]{figures/living17_DOC.pdf}} \hfil
    \subfigure{\includegraphics[width=0.3\linewidth]{figures/living17_linear_fit.pdf}} \hfil   
    \subfigure{\includegraphics[width=0.35\linewidth]{figures/linear_separable_spurious.png}} 
    \vspace{-5pt}
    \caption{\textbf{Left:} Predicted accuracy with DOC on Living17 \breeds~dataset. We observe a substantial gap in the linear fit of same and different subpopulations highlighting poor correlation. \textbf{Middle:} After fitting a robust linear model for DOC on same subpopulation, we show predicted accuracy on different subpopulations with fine-tuned DOC (i.e., DOC (w/ fit)) and compare with ATC without any regression model, i.e., ATC (w/o fit).  While observe substantial improvements in MAE from $24.41$ with DOC (w/o fit) to $13.26$ with DOC (w/ fit), ATC (w/o fit) continues to outperform even DOC (w/ fit) with MAE $10.22$. We show parallel results with other \breeds~datasets in \appref{app:breeeds_ablation}. \textbf{Right :} Empirical validation of our toy model. We show that ATC perfectly estimates target performance as we vary the degree of spurious correlation in target. `$\times$' represents accuracy on source. }
    \vspace{-10pt}
    \label{fig:ablation}
\end{figure}  
  
In \tabref{table:error_estimation}, we report   
MAE results aggregated by 
the nature of the shift in our testbed. 
In \figref{fig:scatter_plot} 
and \figref{fig:intro}(right), we show scatter plots 
for predicted accuracy versus OOD accuracy on 
several datasets. We include 
scatter plots for all datasets and parallel 
results with other architectures in \appref{app:results}. %
In \appref{app:cifar_result}, we also perform ablations on CIFAR using a pre-trained model 
and observe that pre-training doesn't change the efficacy of ATC. 

We predict accuracy on the target
data before and after 
calibration with TS. First, we observe that 
both ATC-NE and ATC-MC (even without TS) obtain 
significantly lower MAE when compared with
other methods (even with TS). 
Note that with TS we observe substantial 
improvements in MAE for all methods.
Overall, ATC-NE (with TS) typically achieves the smallest MAE improving by more than $2\times$ on CIFAR and by $3$--$4\times$ on ImageNet over GDE (the next best alternative to ATC). Alongside, we also observe that a \update{linear fit with robust regression~\citep{siegel1982robust}} on the scatter plot recovers a line close to $x =y$ for ATC-NE with TS while the line is far away from $x=y$ for other methods (\figref{fig:scatter_plot} and \figref{fig:intro}(right)). 
Remarkably, MAE is in the range of $0.4$--$5.8$ with ATC for CIFAR, ImageNet, MNIST, and Wilds. However, MAE is much higher on \textsc{Breeds} benchmark with novel subpopulations. While we observe a small MAE (i.e., comparable to our observations on other datasets) on \textsc{Breeds} with natural and synthetic shifts from the same sub-population, MAE on shifts with novel population is significantly higher with all methods. Note that even on novel populations, ATC continues to dominate all other methods across all datasets in \textsc{Breeds}.

Additionally, for different subpopulations in \breeds~setup, we observe 
a poor linear correlation of the estimated performance with the actual performance as shown in \figref{fig:ablation} (left)(we notice a similar gap in the linear fit for all other methods). Hence in such a setting, we would expect methods that fine-tune a regression model on labeled target examples from shifts with one subpopulation will perform poorly on shifts with different subpopulations. Corroborating this intuition, next, we show that even after fitting a regression model for DOC on natural and synthetic shifts with source subpopulations, ATC without regression model continues to outperform DOC with regression model on shifts with novel subpopulation. 

\textbf{Fitting a regression model on \breeds~with DOC. } 
Using label target data from natural and synthetic shifts for the same subpopulation (same as source), we fit a robust linear regression model~\citep{siegel1982robust} to fine-tune DOC as in \citet{guillory2021predicting}. We then evaluate the fine-tuned DOC (i.e., DOC with linear model) on natural and synthetic shifts from novel subpopulations on \breeds~benchmark. Although we observe significant improvements in the performance of fine-tuned DOC when compared with DOC (without any fine-tuning), ATC without any regression model continues to perform better (or similar) to that of fine-tuned DOC on novel subpopulations (\figref{fig:ablation} (middle)). Refer to \appref{app:breeeds_ablation} for details and \tabref{table:breeds_regression} for MAE on \breeds~with regression model.  %
 










==> ICLR 2022_ Prediction Accuracy on OOD Data/sections/06_theory.tex <==
In this section, we propose 
and analyze a simple theoretical 
model that distills empirical phenomena
from the previous section  
and highlights efficacy of ATC. 
Here, our aim is not to obtain a general 
model that captures complicated real 
distributions on high dimensional input space 
as the images in ImageNet. Instead to further 
our understanding, we focus on an
\emph{easy-to-learn} binary classification task from 
\citet{nagarajan2020understanding}
with linear classifiers, 
that is rich enough to  
exhibit some of the same phenomena
as with deep networks on real data distributions. 

Consider a easy-to-learn binary classification problem with 
two features $x = [x_{\inv}, x_{\spr}] \in \Real^2$ where 
$x_\inv$ is fully predictive 
invariant feature with a margin $\gamma >0$
and $x_\spr \in \{-1, 1\}$ is a spurious feature (i.e., 
a feature that is correlated but
not predictive of the true label). 
Conditional on $y$, the distribution
over $x_\inv$ is 
given as follows: $x_\inv | (y=1)  \sim U[\gamma, c]$ 
and  $x_\inv | (y = 0) \sim U[-c, -\gamma]$, 
where $c$ is a fixed constant greater than $\gamma$. 
For simplicity, we assume that label distribution 
on source is uniform on $\{-1, 1\}$.   
$x_\spr$ is distributed such that 
$P_s[ x_\spr \cdot (2y-1) > 0] = p_\spr $, where 
$p_\spr \in (0.5, 1.0)$ controls 
the degree of spurious correlation. 
To model distribution shift, 
we simulate target data with different
degree of spurious correlation, i.e., in target distribution 
$P_t[ x_\spr \cdot (2y-1) > 0] = p_\spr^\prime \in [0,1]$.  
Note that here we do not consider shifts in the label 
distribution but our result extends to arbitrary shifts 
in the label distribution as well. 

In this setup, we examine linear sigmoid classifiers of the form  
$f(x) = \left[ \frac{1}{1 + e^{w^T x}}, \frac{ e^{w^T x}}{1 + e^{w^T x}}\right]$
where $w = [w_{\inv}, w_\spr] \in \Real^2$. 
While there exists a linear classifier with 
$w = [1,0]$ that correctly classifies all the points
with a margin $\gamma$,  \citet{nagarajan2020understanding}
demonstrated that a linear classifier will 
typically have a dependency on the spurious feature, 
i.e., $w_\spr \ne 0$. They show that due to geometric skews, 
despite having positive dependencies on the invariant feature, 
a max-margin classifier trained on finite samples
relies on the spurious feature. 
Refer to \appref{app:toy_model} 
for more details on these skews. 
In our work, we show that given a linear classifier 
that relies on the spurious feature 
and achieves a non-trivial performance on 
the source (i.e., $w_\inv > 0$),  
ATC with maximum confidence score function  
\emph{consistently}
estimates the accuracy on the target distribution. 

\begin{theorem}[Informal] \label{thm:toy_theory}
Given any classifier with $w_\inv > 0$ in the above setting, 
the threshold obtained in \eqref{eq:ATC_thres} together with 
ATC as in \eqref{eq:ATC_pred}
with maximum confidence score function
obtains a consistent estimate of the target accuracy. 
\end{theorem}

Consider a classifier that depends positively 
on the spurious feature (i.e., $w_{\spr} > 0$). 
Then as the spurious correlation 
decreases in the target data, 
the classifier accuracy on the target will drop and 
vice-versa if the spurious correlation increases on the target data. 
\thmref{thm:toy_theory} shows that the threshold identified with 
ATC as in \eqref{eq:ATC_thres} remains invariant as the distribution shifts
and hence ATC as in \eqref{eq:ATC_pred}
will correctly estimate the 
accuracy with shifting distributions. 
Next, we illustrate \thmref{thm:toy_theory} 
by simulating the setup empirically. 
First we pick a arbitrary classifier
(which can also be obtained by training 
on source samples), 
tune the threshold on hold-out source examples 
and predict accuracy with different methods as
we shift the distribution by varying the degree 
of spurious correlation. 

\textbf{Empirical validation and comparison with other methods. {} {}}
\figref{fig:ablation}(right) shows that as the degree of spurious correlation varies,
our method accurately estimates the target performance where  
all other methods fail to accurately estimate the target performance. 
Understandably, due to poor calibration of the sigmoid linear 
classifier AC, DOC and GDE fail. While in principle IM 
can perfectly estimate the accuracy on target in this case, 
we observe that it is highly sensitive to the number bins and choice of 
histogram binning (i.e., uniform mass or equal width binning).
We elaborate more on this in \appref{app:toy_model}.  %


\textbf{Biased estimation with ATC. {} {}} 
Now we discuss changes in the above 
setup where ATC yields 
inconsistent estimates. 
We assumed that both in 
source and target $x_{\inv}|y=1$ 
is uniform between $[\gamma, c]$ 
and $x|y=-1$ is uniform 
between $[-c, -\gamma]$. 
Shifting the support of target class 
conditional $p_t(x_{\inv}|y)$ may 
introduce a bias in ATC estimates, e.g.,  
shrinking the support to 
$c_1$($<c$) (while maintaining 
uniform distribution) 
in the target will lead to an over-estimation 
of the target performance with ATC.  
In \appref{app:general_result}, %
we elaborate on this 
failure and present a general
(but less interpretable)  
classifier dependent distribution shift 
condition where ATC is guaranteed to yield consistent 
estimates.



==> ICLR 2022_ Prediction Accuracy on OOD Data/sections/07_conclusion.tex <==
In this work, we proposed ATC, a simple method for 
estimating target domain accuracy 
based on unlabeled target 
(and labeled source data).
ATC achieves remarkably low estimation error 
on several synthetic and natural shift benchmarks 
in our experiments. 
Notably, our work draws inspiration from recent 
state-of-the-art methods that use softmax confidences 
below a certain threshold for OOD detection~\citep{hendrycks2016baseline,hendrycks2019scaling}   
and takes a step forward in answering questions
raised in \citet{deng2021labels} 
about the practicality of threshold based methods.   

Our distribution shift toy model justifies ATC 
on an easy-to-learn binary classification task. 
In our experiments, we also observe
that calibration significantly improves estimation with ATC. 
Since in binary classification, post hoc calibration with TS 
does not change the effective threshold, 
in future work, we hope to extend our theoretical model 
to multi-class classification to understand the efficacy of calibration. 
Our theory establishes that a classifier's accuracy 
is not, in general identified, from labeled source 
and unlabeled target data alone, 
absent considerable additional constraints
on the target conditional $p_t(y|x)$.
In light of this finding, 
we also hope to extend our understanding 
beyond the simple theoretical toy model
to characterize broader sets of conditions 
under which ATC might be guaranteed %
to obtain consistent estimates. 
Finally, we should note that
while ATC outperforms previous approaches, 
it still suffers from large estimation error
on datasets with novel populations, e.g., \breeds. 
We hope that our findings can lay the groundwork 
for future work for improving accuracy estimation on such datasets. 

